SicHash -- Small Irregular Cuckoo Tables for Perfect Hashing

A Perfect Hash Function (PHF) is a hash function that has no collisions on a given input set. PHFs can be used for space efficient storage of data in an array, or for determining a compact representative of each object in the set. In this paper, we present the PHF construction algorithm SicHash - Small Irregular Cuckoo Tables for Perfect Hashing. At its core, SicHash uses a known technique: It places objects in a cuckoo hash table and then stores the final hash function choice of each object in a retrieval data structure. We combine the idea with irregular cuckoo hashing, where each object has a different number of hash functions. Additionally, we use many small tables that we overload beyond their asymptotic maximum load factor. The most space efficient competitors often use brute force methods to determine the PHFs. SicHash provides a more direct construction algorithm that only rarely needs to recompute parts. Our implementation improves the state of the art in terms of space usage versus construction time for a wide range of configurations. At the same time, it provides very fast queries.

==> Makefile <==
paper_size ?= a4
pdf_quality ?= printer

all: paper

clean:
	rm -rf paper.pdf
	rm -rf *.log *.aux *.bbl *.blg .toc *.out *.toc
	rm -rf rev.tex

RERUN = '(There were undefined references|Rerun to get (cross-references|the bars) right)'
RERUNBIB = 'No file.*\.bbl|Citation.*undefined'
UNDEFINED = '((Reference|Citation).*undefined)|(Label.*multiply defined)'

pdflatex = pdflatex -interaction=batchmode paper.tex
pdflatex_safe = (pdflatex -interaction=batchmode paper.tex || true)
bibtex = bibtex paper

paper:: *.tex
	@echo "====> LaTeX first pass"
	$(pdflatex) || cat paper.log
	@if egrep -q $(RERUNBIB) paper.log ; then echo "====> BibTex" && $(bibtex) && echo "====> LaTeX BibTeX pass" && $(pdflatex_safe) ; fi
	@if egrep -q $(RERUN) paper.log ; then echo "====> LaTeX rerun" && $(pdflatex_safe); fi;
	@if egrep -q $(RERUN) paper.log ; then echo "====> LaTeX rerun" && $(pdflatex_safe); fi;
	@echo "====> Undefined references and citations:"
	@egrep -i $(UNDEFINED) paper.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" paper.log || echo "None."

